Suzaku Observations of Moderately Obscured (Compton-thin) Active Galactic Nuclei Selected by Swift/BAT Hard X-ray Survey

We report the results obtained by a systematic, broadband (0.5--150 keV) X-ray spectral analysis of moderately obscured (Compton-thin; $22 \leq \log N_{\rm H} < 24$) active galactic nuclei (AGNs) observed with Suzaku and Swift/Burst Alert Telescope (BAT). Our sample consists of 45 local AGNs at $z<0.1$ with $\log L_{\rm 14-195\1mmkeV} > 42$ detected in the Swift/BAT 70-month survey, whose Suzaku archival data are available as of 2015 December. All spectra are uniformly fit with a baseline model composed of an absorbed cutoff power-law component, reflected emission accompanied by a narrow fluorescent iron-K$\alpha$ line from cold matter (torus), and scattered emission. Main results based on the above analysis are as follows. (1) The photon index is correlated with Eddington ratio, but not with luminosity or black hole mass. (2) The ratio of the iron-K$\alpha$ line to X-ray luminosity, a torus covering fraction indicator, shows significant anti-correlation with luminosity. (3) The averaged reflection strength derived from stacked spectra above 14 keV is larger in less luminous ($\log L_{\rm 10-50\1mmkeV} \leq 43.3$; $R= 1.04^{+0.17}_{-0.19}$) or highly obscured AGNs ($\log N_{\rm H} > 23$; $R = 1.03^{+0.15}_{-0.17}$) than in more luminous ($\log L_{\rm 10-50\1mmkeV} > 43.3$; $R= 0.46^{+0.08}_{-0.09}$) or lightly obscured objects ($\log N_{\rm H} \leq 23$; $R = 0.59^{+0.09}_{-0.10}$), respectively. (4) The [O IV] 25.89 $\mu$m line to X-ray luminosity ratio is significantly smaller in AGNs with lower soft X-ray scattering fractions, suggesting that the [O IV] 25.89 $\mu$m luminosity underestimates the intrinsic power of an AGN buried in a small opening-angle torus.

==> info_ave_spec.tex <==
% TABLE.1 
%%%%%%%%%
\begin{landscape}
\LongTables
\begin{deluxetable}{cccccccccccccccccccc}
\tabletypesize{\scriptsize}
\tabletypesize{\footnotesize}
\setlength{\tabcolsep}{0.01in}
\tablecaption{Information of detected emission/absorption lines\label{tab:info_lines}}
\tablewidth{-0.5pt}
\tablehead{\colhead{Target Name} 
& \colhead{$N_{\rm 6.4\hspace{1mm}keV}$}  
& \colhead{$N_{\rm 6.31\hspace{1mm}keV}$}  
& \colhead{$N_{\rm 6.68\hspace{1mm}keV}$}  
& \colhead{$N_{\rm 6.93\hspace{1mm}keV}$}  
& \colhead{$N_{\rm 7.06\hspace{1mm}keV}$}  
& \colhead{$N_{\rm 7.48\hspace{1mm}keV}$}  
& \colhead{$E_{1}$}  & \colhead{$N_{1}$}  
& \colhead{$E_{2}$}  & \colhead{$N_{2}$}  
& \colhead{$E_{3}$}  & \colhead{$N_{3}$}  \\ 
\colhead{(1)} & \colhead{(2)} & \colhead{(3)} & \colhead{(4)} &
\colhead{(5)} & \colhead{(6)} & \colhead{(7)} & \colhead{(8)}  & \colhead{(9)} &
\colhead{(10)} & \colhead{(11)}  & \colhead{(12)} & \colhead{(13)} 
} 
\startdata
\thispagestyle{empty}
 NGC 1142 &  $ 20.4^{+1.4}_{-1.3}  $ &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - \\ 
 2MASX J0318+6829 &  $ 2.9\pm0.9  $ &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - \\ 
 2MASX J0350-5018 &  $ 5.6\pm1.0  $ &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - \\ 
 2MASX J0444+2813 &  $ 8.9\pm0.9  $ &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - \\ 
 2MASX J0505-2351 &  $ 8.8\pm1.0  $ &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - \\ 
 ESO 005-G004 &  $ 19.6\pm1.6  $ &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - \\ 
 2MASX J0911+4528 &  $ 2.0\pm0.7  $ &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - \\ 
 2MASX J1200+0648 &  $ 7.3^{+-7.3}_{-7.3}  $ &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - \\ 
 Mrk 1498 &  - &  - &  - &  - &  - &  - & $ 6.29^{0.02}_{-0.02}  $ & $ 10.6\pm1.9  $ &  - &  - &  - &  - \\ 
 UGC 03142 &  $ 13.3\pm1.3  $ &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - \\ 
 UGC 12741 &  $ 5.5^{+-5.5}_{-5.5}  $ &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - &  - 
\enddata 
\tablecomments{
(1) Galaxy name. 
(2)-(7) Normalization of emission lines at 6.40 keV, 6.31 keV, 6.68 keV, 6.93 keV, 7.06 keV, and 7.48 keV in the units of 
$\times10^{-6}$ photons cm$^{-2}$ s$^{-1}$. 
(8)-(13) Line Energy and normalization of emission/absorption lines in the units of keV and $\times10^{-6}$ photons cm$^{-2}$ s$^{-1}$. 
 }
\end{deluxetable}
\clearpage
\end{landscape}

